Stochastic Gradient Descent Optimizes Over-parameterized Deep ReLU Networks

We study the problem of training deep neural networks with Rectified Linear Unit (ReLU) activation function using gradient descent and stochastic gradient descent. In particular, we study the binary classification problem and show that for a broad family of loss functions, with proper random weight initialization, both gradient descent and stochastic gradient descent can find the global minima of the training loss for an over-parameterized deep ReLU network, under mild assumption on the training data. The key idea of our proof is that Gaussian random initialization followed by (stochastic) gradient descent produces a sequence of iterates that stay inside a small perturbation region centering around the initial weights, in which the empirical loss function of deep ReLU networks enjoys nice local curvature properties that ensure the global convergence of (stochastic) gradient descent. Our theoretical results shed light on understanding the optimization for deep learning, and pave the way for studying the optimization dynamics of training modern deep neural networks.

==> sgd_converge.tex <==

\section{Convergence of Stochastic Gradient Descent}
\begin{theorem}\label{thm:SGD}
Under Assumptions \ref{assump:loss}-\ref{assump:m_scaling}.  At the initialization, for each $l\in[L]$, let  $\wb^{(0)}_{l,1},\ldots,\wb^{(0)}_{l,m_{l}}$ be generated independently from $N(\mathbf{0},2\Ib/m_l)$. Then we have the following results on the minimum required number of hidden nodes $m$ and iteration number $K$ such that with constant probability, the stochastic gradient can find a point $\Wb^{(best)}$ within the iteration sequence $\{\Wb^{(k)}\}_{k=0,1,\dots,K}$ satistying $L_S(\Wb^{(best)})\le \epsilon$,
\begin{align*}
m=\left\{\begin{array}{ll}
 \text{poly}(n,\phi^{-1})\cdot \epsilon^{-4p}\cdot e^{-O(L)}& 0\le p <\frac{1}{2}\\
\text{poly}(n,\phi^{-1})\cdot\log^2(1/\epsilon)\cdot e^{-O(L)}& p=\frac{1}{2}\\
\text{poly}(n,\phi^{-1})\cdot\epsilon^{2-4p}\cdot e^{-O(L)}& \frac{1}{2}<p \le 1,
\end{array} \right.
\end{align*}
and 
\begin{align*}
K=\left\{\begin{array}{ll}
 \text{poly}(n,\phi^{-1})\cdot \epsilon^{-2p}\cdot e^{-O(L)}& 0\le p <\frac{1}{2}\\
\text{poly}(n,\phi^{-1})\cdot\log(1/\epsilon)\cdot e^{-O(L)}& p=\frac{1}{2}\\
\text{poly}(n,\phi^{-1})\cdot\epsilon^{1-2p}\cdot e^{-O(L)}& \frac{1}{2}<p \le 1.
\end{array} \right.
\end{align*}
\end{theorem}








% \begin{lemma}\label{lemma:lip_GD_sparse}
% With high probability
% \begin{align*}
% \bigg\|\vb^\top\bigg(\prod_{r=l+1}^L\bSigma_{r,i}^{(k)}\Wb_{r}^{(k)\top}\bigg)\tilde \bSigma_{l,i}^{(k+1)}\bigg\|_2\le \sqrt{s\log(M)}.
% \end{align*}
% \end{lemma}






\subsection{Proof of Theorem \ref{thm:SGD}}
\begin{lemma}[Convergence rate]\label{lemma:convergence_SGD_nonlinear}
Suppose that for all $l\in[L]$, $\Wb_{l}$ is randomly generated from Gaussian distribution $N(\mathbf{0}, m_l \Ib/2)$ respectively. If the step size $\eta  = O(n^{-6}BM^{-1}\phi^3)\cdot e^{-O(L)}$ and the perturbation level $\tau = \tilde O(n^{-15}\phi^9)\cdot e^{-O(L)}$, the stochastic gradient can find a point $\Wb^{(best)}$ along the iteration sequence $\{\Wb^{(i)}\}_{i=1,\dots,K}$ such that with constant probability the training loss $L_S(\Wb^{(best)})\le \epsilon$ if the following holds for $K\eta$,
\begin{align*}
K\eta =\left\{\begin{array}{ll}
O\big(n^{7-2p}\epsilon^{-2p}/(m\phi^3)\big)& 0\le p <\frac{1}{2}\\
O\big(n^6\log(1/\epsilon)/(m\phi^3)\big)& p=\frac{1}{2}\\
O\big(n^{7-2p}\epsilon^{1-2p}/(M\phi^3)\big)& \frac{1}{2}<p \le 1
\end{array} \right.  
\end{align*}
when $x_0= -\infty$, and
\begin{align*}
K\eta =  O\big(n^{7-2p}\epsilon^{-2p}/(m\phi^3)\big)
\end{align*}
when $x_0 > -\infty$, 
then with high probability the gradient descent finds an point $\Wb^{(k)}$ such that $L_S(\Wb)\le\epsilon$.
\end{lemma}
\begin{proof}[Proof of Theorem \ref{thm:SGD}]
The proof for $K$ is straightforward. Utilizing the results of $K\eta$ and $\eta$ provided in Lemma \ref{lemma:convergence_SGD_nonlinear} directly yields the bounds on the iteration number $K$.

In terms of the minimum required number of hidden nodes, i.e., $m$,  the proof resembles that of Theorem \ref{thm:GD}. Specifically, we first derive the upper bound of $\|\Wb_l^{(k)}-\Wb_l^{(0)}\|_2$ and show that it is upper bounded by the preset perturbation level $\tau$. Note that during the stochastic gradient descent, we have
\begin{align*}
\|\Wb_l^{(k)} - \Wb_l^{(0)}\|_2\le \|\Wb_l^{(k)}-\Wb_l^{(0)}\|_2\le \eta \sum_{i=0}^{k-1}\|\gb_{l}^{(k)}\|_2,
\end{align*}
where $\gb_{l}^{(k)}$ is the stochastic partial gradient with respect to $\Wb_l$ in the $k$-th iteration. Then by Lemma \ref{lemma:upper_grad} and Assumption \ref{assump:Lipschitz}, we have
\begin{align*}
\|\gb_l^{(k)}\|_2 \le 4^LM^{1/2}\rho,
\end{align*}
which implies that 
\begin{align*}
\|\Wb_l^{(k)} - \Wb_l^{(0)}\|_2\le 4^LM^{1/2}\rho k\eta .   
\end{align*}
Note that $\tau = \tilde O(n^{-15\phi^9})\cdot e^{-O(L)}$. Then we are able to derive the lower bound of $m$ by solving $4^LM^{1/2}\rho k\eta\le \tau$. Using the results of $k\eta$ presented in Lemma \ref{lemma:convergence_SGD_nonlinear}, we have the following results on $m$:
\begin{itemize}
    \item $x_0=-\infty$:
\begin{align*}
M=\left\{\begin{array}{ll}
\tilde O\big(n^{44-4p}/\phi^{24}\big)\cdot e^{-O(L)}& 0\le p <\frac{1}{2}\\
\tilde O\big(n^{42}\log^2(1/\epsilon)/\phi^{24}\big)\cdot e^{-O(L)})& p=\frac{1}{2}\\
\tilde O\big(n^{44-4p}\epsilon^{2-4p}/\phi^{24}\big)\cdot e^{-O(L)}& \frac{1}{2}<p \le 1,
\end{array} \right.
\end{align*}
\item $x_0 > -\infty$
\begin{align*}
M=\tilde O\big(n^{44-4p}/\phi^{24}\big)\cdot e^{-O(L)}.
\end{align*}
\end{itemize}
\end{proof}
